A Coupled Optimization Framework for Correlated Equilibria in Normal-Form Game

In competitive multi-player interactions, simultaneous optimality is a key requirement for establishing strategic equilibria. This property is explicit when the game-theoretic equilibrium is the simultaneously optimal solution of coupled optimization problems. However, no such optimization problems exist for the correlated equilibrium, a strategic equilibrium where the players can correlate their actions. We address the lack of a coupled optimization framework for the correlated equilibrium by introducing an {unnormalized game} -- an extension of normal-form games in which the player strategies are lifted to unnormalized measures over the joint actions. We show that the set of fully mixed generalized Nash equilibria of this unnormalized game is a subset of the correlated equilibrium of the normal-form game. Furthermore, we introduce an entropy regularization to the unnormalized game and prove that the entropy-regularized generalized Nash equilibrium is a sub-optimal correlated equilibrium of the normal form game where the degree of sub-optimality depends on the magnitude of regularization. We prove that the entropy-regularized unnormalized game has a closed-form solution, and empirically verify its computational efficacy at approximating the correlated equilibrium of normal-form games.

==> contents/ce_gne_equivalence_new_version.tex <==
\section{Lifting correlated equilibrium to generalized Nash equilibrium}
While a correlated equilibrium has the interpretation of being a `simultaneously optimal' strategy in literature, this interpretation lacks an explicit optimization formulation like the one that exists for Nash equilibrium in the form of~\eqref{eqn:ne_optimization}. In this section, we formulate a novel game in which the player strategy spaces are lifted from the probability measure space over $[A_{i}]$ to the unnormalized measure space over $[A] = \prod_{i\in[N]} [A_i]$. We show that a fully mixed correlated strategy is a correlated equilibrium of the normal form game if and only if it corresponds to a generalized Nash equilibrium of the lifted game over unnormalized measures. 

\subsection{Unnormalized measures}
We first consider a relaxation of probability distributions to unnormalized measures with finite mass~\cite{swendsen2014unnormalized,frogner2015learning}. 
\begin{definition}[Unnormalized measure]\label{def:unnormal_strategy}
Given an action set $[A]$ and a corresponding strategy set $\Delta_A$, the vector $\alpha \in \reals_+^{A}$ is an unnormalized measure over the sample space $[A]$ if $\alpha(a) \geq 0$ for all $a \in [A]$, and there exists $M \in \reals_+$ such that $\frac{1}{M}\alpha \in \Delta_A$.  
\end{definition}
Given two unnormalized measures $\alpha_1, \alpha_2$ over the same action space, we denote their \textbf{element-wise product} by $\alpha_1 \circ\alpha_2$, such that 
\[(\alpha_1 \circ\alpha_2) \in \reals_+^{A}, (\alpha_1 \circ\alpha_2)(a) = \alpha_1(a)\alpha_2(a), \ \forall a \in [A].\] 
We consider decompositions of the correlated strategy $y$ (Definition~\ref{def:c_strategy})  into $N$ unnormalized measures. 
\begin{definition}[Normalized Decomposition]\label{def:decompose_ce} Given a correlated strategy $y \in \Delta_A$, we say that $(\alpha_1,\ldots,\alpha_N)$ is a normalized decomposition of $y$ and $y$ is a product of $(\alpha_1,\ldots\alpha_N)$ if 
\begin{equation}\label{eqn:decomposing_y}
   y = \alpha_1\circ\ldots\circ\alpha_N, \ \alpha_i \in \reals^A_+, \ \forall i \in [N]. 
\end{equation}
\end{definition}
The mapping $y\mapsto (\alpha_1,\ldots,\alpha_N)$ is surjective but not injective. Every correlated strategy has at least one valid decomposition, but multiple sets of unnormalized measures can produce the same correlated strategy. 
\begin{lemma}\label{lem:support_inv}
    Every correlated strategy $y \in \Delta_A$ has an infinite number of decomposition's in the form of~\eqref{eqn:decomposing_y}. Furthermore, if $(\alpha_1,\ldots,\alpha_N)$ satisfies
    \begin{equation}\label{eqn:support_constraint}
        \ones^\top(\alpha_1 \circ \ldots\circ\alpha_N) = 1,   \alpha^i \geq 0, \ \forall i \in [N],
    \end{equation}
    then $y = \alpha^1 \circ \ldots\circ\alpha^N$ is a correlated strategy. 
\end{lemma}
\begin{proof}
    Consider the unnormalized measures $(\alpha_1,\ldots,\alpha_N)$ that satisfy~\eqref{eqn:support_constraint} and let $y =\alpha_1\circ\ldots\circ\alpha_N$, then $y$ is a correlated strategy as defined in Definition~\ref{def:c_strategy}. To show that every correlated strategy $y$ has an infinite number of decomposition's, we first show there exist at least one feasible decomposition: $\alpha_1 = y$, $\alpha_j = \ones$ for all $j \neq 1$. We then select $d\in \reals$, $d > 0$ and define the measures $\hat\alpha_1 = d\alpha_1$, $\hat\alpha_2 = \frac{1}{d}\alpha_2$, and $\hat\alpha_{j} = \alpha_j$ for all $j\notin \{1,2\}$, then the product of $(\hat\alpha_1,\hat\alpha_2,\ldots\circ\hat\alpha_N)$ satisfies $y =\hat\alpha_1\circ\hat\alpha_2\ldots,\hat\alpha_N$. Since we can select arbitrary positive real number $d$, there exist an infinite number of decomposition's.  
\end{proof}
\begin{example}[Normalized decompositions]\label{ex:unnnormalized_distributions}
In a two player, finite action game where $A_1 = A_2 \in\mathbb{N}$. We represent the unnormalized measures by $A_1\times A_2$-dimensional matrices, $\alpha \in \reals^{A_1\times A_2}$, such that any element-wise product $\alpha_i\circ\alpha_j$ is equivalent to the Hadarmard product between their matrix counterparts. The following are all valid normalized decomposition's and their correlated strategy product.
\begin{equation}\label{eqn:decomposition_NE}
    \left\{\begin{pNiceMatrix}[last-row]
0 & 0 & 0 \\
1 & 1 & 1 \\
 0 & 0 & 0\\
       & \alpha_1    &
\end{pNiceMatrix},  \ \begin{pNiceMatrix}[last-row]
0 & 0 & 1 \\
0& 0& 1 \\
 0 & 0 & 1\\
       & \alpha_2    &
\end{pNiceMatrix}\right\}, \begin{pNiceMatrix}[last-row]
0 &0 & 0 \\
0& 0& 1 \\
 0 & 0 & 0\\
       & y_{\alpha}    &
\end{pNiceMatrix},
\end{equation}
\begin{equation}\label{eqn:decomposition_positive}
   \left\{\frac{1}{45}\begin{pNiceMatrix}[last-row]
1 & 1 & 1 \\
1 & 1 & 1 \\
1 & 1 & 1\\
       & \beta_1    &
\end{pNiceMatrix},  \ \begin{pNiceMatrix}[last-row]
1 & 2 & 3 \\
4& 5& 6 \\
 7 & 8 & 9\\
       & \beta_2    &
\end{pNiceMatrix}\right\}, \frac{1}{45}\begin{pNiceMatrix}[last-row]
1 & 2 & 3 \\
4& 5& 6 \\
 7 & 8 & 9\\
       & y_{\beta}    &
\end{pNiceMatrix},  
\end{equation}
\begin{equation}\label{eqn:decomposition_non_invariant}
    \left\{\begin{pNiceMatrix}[last-row]
0 & 0 & 0 \\
0 & 0 & 1 \\
0 & 1 & 0\\
       & \gamma_1    &
\end{pNiceMatrix},  \ \half\begin{pNiceMatrix}[last-row]
1 & 0 & 0 \\
0& 1& 1 \\
 0 & 1 & 1\\
       & \gamma_2    &
\end{pNiceMatrix}\right\},  \frac{1}{2}\begin{pNiceMatrix}[last-row]
0 &0 & 0 \\
0& 1& 0 \\
 0 & 0 & 1\\
       & y_{\gamma}    &
\end{pNiceMatrix}.
\end{equation}
\end{example}

\subsection{Unnormalized game} 
We define an \textbf{unnormalized game} as the following extension of the normal-form game presented in Section~\ref{sec:prelim}: instead of choosing probability distributions supported on each player's individual action space, each player $i$ to chooses an unnormalized measure $\alpha_i$ over the joint action space $[A]$ as defined in Definition~\ref{def:unnormal_strategy}, constrained by the condition that the product $y = \alpha_1\circ\ldots\alpha_N$ is a correlated strategy. The player objectives remain the expected cost incurred by each player~\eqref{eqn:cost_overloading}, which is a multi-linear function of the unnormalized measures through~\eqref{eqn:decomposing_y} and~\eqref{eqn:cost_overloading}.
\begin{equation}\label{eqn:ce_individual_opt}
\begin{aligned}
    \min_{\alpha_i\in \reals_+^{A}} & \sum_{a \in [A]} {\ell}_i(a) \alpha_1(a)\ldots\alpha_N(a), \\
    \mbox{s.t. } &\sum_{a_i \in [A_i]}(\alpha_1\circ \ldots\circ\alpha_N)(a_i, a_{-i}) = \frac{1}{A_{-i}},  \ \forall a_{-i} \in [A_{-i}] \\ %\frac{1}{A_{-i}}
    & \alpha_i(a) \geq 0, \ \forall a \in [A]. %\ones^\top \alpha = \ones^\top,
\end{aligned}
\end{equation}
In the unnormalized game, each player's strategy  $\alpha_i$ has the same dimension as the correlated strategy of the original finite game. Given the opponents' strategies $\alpha_{-i}$, player $i$ uses their strategy $\alpha_i$ to optimize the expected cost $\sum_{a \in [A]} {\ell}_i(a) \alpha_1(a)\ldots\alpha_N(a)$, constrained by a mass constraint at each opponent joint strategy $a_{-i}$: $\sum_{a_i \in [A_i]}(\alpha_1\circ \ldots\circ\alpha_N)(a_i, a_{-i}) = \frac{1}{A_{-i}}$. 
% We say that $\alpha_i$ is the best response to opponent strategies $\alpha_{-i}$ if $\alpha^i$ is in the argmin set of~\eqref{eqn:ce_individual_opt}.  
The optimal solution of this game is a generalized Nash equilibrium, where, in addition to minimizing their expected cost, each player's strategy must be feasible with respect to their opponent's strategies. 
\begin{definition}[Generalized Nash equilibrium]\label{def:gNE}
    A joint strategy $(\alpha_1^\star,\ldots, \alpha_N^\star)$ is a generalized Nash equilibrium if for all $i \in [N]$,
    $\alpha^\star_i$ is the optimal solution to~\eqref{eqn:ce_individual_opt}.
\end{definition}
A generalized Nash equilibrium extends the standard Nash equilibrium (Definition~\ref{def:CE}) to games where each player's strategy feasibility depends on the opponents' strategies. In the unnormalized game, all players share the strategy constraint given by~\eqref{eqn:support_constraint}. Next, we restrict our analysis to fully mixed unnormalized measures and show that when a set of fully mixed unnormalized measures forms a generalized Nash equilibrium, their product is a correlated equilibrium.  
\begin{assumption}[Fully mixed correlated strategies]\label{assum:support invariance} A measure $\alpha \in \reals_+^{A}$ is fully mixed if for all $a \in [A]$, $\alpha(a) > 0$. 
\end{assumption}
When a correlated strategy is fully mixed, all of its normalized decomposition's $(\alpha_1,\ldots,\alpha_N)$ satisfy Assumption~\ref{assum:support invariance}. 
% Normalized decompositions that satisfy Assumption~\ref{assum:support invariance} are also deterministic: given $\alpha_{-i}$ and $y$, there exist a unique $\alpha_i$ such that $(\alpha_1,\ldots, \alpha_N)$ is a feasible decomposition of $y$. 
Games with certain player cost structures, such as zero sum games and games with non-dominant strategies, tend to have fully mixed Nash and correlated equilibrium~\cite{solan2002correlated,reny1999existence}. 
\subsection{Equivalence between gNE and correlated equilibrium}
For fully mixed correlated strategies $y$ with a normalized decomposition $(\alpha_1,\ldots,\alpha_N)$, we can show that $y$ is a correlated equilibrium of the normal form game if and only if $(\alpha_1,\ldots,\alpha_N)$ is a generalized Nash equilibrium of the unnormalized  game. 
\begin{proposition}\label{prop:ce_necessary}
    If $(\alpha_1,\ldots,\alpha_N)$ is the generalized Nash equilibrium (Definition~\ref{def:gNE}) of the unnormalized game~\eqref{eqn:ce_individual_opt}, and the $\alpha_{i}$'s satisfy Assumption~\ref{assum:support invariance}, then the product $y = \alpha_1\circ\ldots\circ\alpha_N$ is a correlated equilibria of the normal form game~\eqref{eqn:ce}.
\end{proposition}
\begin{proof}
We prove this proposition by showing that when satisfied together, Assumption~\ref{assum:support invariance} and the coupled KKT conditions of~\eqref{eqn:ce_individual_opt} imply the correlated equilibrium condition in~\eqref{eqn:ce}.
From~\cite{facchinei2009generalized}, the coupled KKT conditions of~\eqref{eqn:ce_individual_opt} are necessary for $(\alpha_1,\ldots,\alpha_N)$ to be a generalized Nash equilibrium of the unnormalized game. Therefore, we show that~\eqref{eqn:ce} holds for $y = \alpha_1\circ\ldots\circ\alpha_N$ for all the KKT points $(\alpha_1,\ldots\alpha_N)$ of~\eqref{eqn:ce_individual_opt}. 

From the unnormalized game~\eqref{eqn:ce_individual_opt} for player $i$, we assign the Lagrange multipliers $\sigma_{i }(a_{-i}) \in \reals$ for the constraints $\sum_{a_i\in[A_i]}(\alpha_1\circ\ldots\circ\alpha_N)(a_i, a_{-i}) = 1/A_{-i}$ and $\mu_{i}(a)$ for the constraints $\alpha_{i}(a)\geq 0$. The first order gradient condition and the complementarity condition of the KKT are given by 
    \begin{multline}
        \ell_i(a) \alpha_{-i}(a) - \sigma_{i}(a_{-i}) \alpha_{-i}(a) - \mu_{i}(a) = 0,  \\ \mu_{i}(a) = \begin{cases}
        \geq 0 & \alpha_{i}(a) = 0\\
        = 0 & \alpha_{i}(a) > 0
    \end{cases},\forall (i,a) \in [N]\times [A].
    \end{multline}
When $\alpha_{-i}(a) > 0$, the KKT conditions above imply that
\begin{equation}
    \ell_i(a) \begin{cases}
     = \sigma_{i}(a_{-i}), & \text{if }\alpha_{i}(a) > 0 \\
    \geq \sigma_{i}, & \alpha_i(a) = 0 
\end{cases}, \ \forall (i,a) \in [N]\times[A].
\end{equation}
% We can conclude that $(\ell_i(a) - \lambda)\alpha_{-i}(a) \geq 0$ for all $a \in [A]$, and that the inequality is strict when $\alpha_i(a) > 0$. 

From Assumption~\ref{assum:support invariance}, $\alpha_{-i}(a) > 0$ and $\alpha_{i}(a) > 0$ for all $a \in [A]$. Therefore, $\mu_i(a) = 0$, $\sigma_{i}(a_{-i}) = \ell_i(a_i, a_{-i})$ for all $a_i \in [A_i]$. In particular, $\ell_i(a_i, a_{-i}) = \ell_i(\hat{a}_i, a_{-i})$ for all $a_i, \hat{a}_i \in [A_i]$. The correlated equilibrium condition~\eqref{eqn:ce} $(\ell_i(a_{i}, a_{-i}) - \ell_i(\hat{a}_i, a_{-i}))y(a_i, a_{-i})$ will then evaluate strictly to $0$ for all $\hat{a}_i \in [A_i]$ and $i \in [N]$.
We conclude that $y = \alpha_{1}\circ\ldots\circ\alpha_{N}$ is a correlated equilibrium.
\end{proof}
\begin{remark}
Proposition~\ref{prop:ce_necessary} suggests that a correlated equilibrium is fully mixed only if $\ell_{i}(a_i, a_{-i}) $ evaluates to the same value for all $a_i\in[A_i]$. While this may seem restrictive, we use entropy regularizations to in Section~\ref{sec:entropy_reg_equilibria} to produce games in which the regularized costs are all equal for each opponent action $a_{-i}$. We can show that the generalized Nash equilibrium under regularization will approximate the correlated equilibrium of a normal form game without any restrictions on the cost structure.  
\end{remark}
The reverse of Proposition~\ref{prop:ce_necessary} is not true: if $y$ is a fully mixed correlated equilibrium, then its normalized decomposition is a generalized Nash equilibrium of the unnormalized game. 
\begin{example}[Correlated equilibria not captured by unnormalized game]
Consider the $2\times 2$ matrix game where player one chooses the row and player two chooses the column. The player costs are given by matrices $A$ and $B$, respectively, defined as 
\[P_1 = \begin{bmatrix}
    3& 3 \\ 2 &4
\end{bmatrix}, \ P_2 =  \begin{bmatrix}
    1& 2 \\ 1 &0
\end{bmatrix}.\]
We vectorize the joint action space to be $[A] = \{a_1, a_2, a_3, a_4\}$, corresponding to the counterclockwise sequence of joint actions in matrix $P_i$ starting from the top left. For $y \in \Delta_4$ to be a correlated equilibrium as defined in~\eqref{eqn:ce}, it must satisfy
\begin{equation}\label{eqn:bimatrix_ce}
 \begin{aligned}
    3y(a_1) + 3 y(a_4) - 2y(a_2) - 4 y(a_3) &\leq 0\\
    1 y(a_1) + 1 y(a_2) - 0 y(a_3) - 2 y(a_4) &\leq 0
\end{aligned}   
\end{equation}
We can verify that $y_{CE} = \begin{bmatrix}
    \frac{1}{4} & \frac{1}{4} & \frac{1}{4} & \frac{1}{4}
\end{bmatrix}$ satisfies~\eqref{eqn:bimatrix_ce}. The unnormalized game played is given by
\begin{equation}\label{eqn:bimatrix_gne}
    \begin{aligned}
        \min_{\alpha_1} & \half \Big(3\alpha_1(a_1) + 2\alpha_1(a_2) + 4 \alpha_1(a_3) + 4\alpha_1(a_4)\Big) \\
        \mbox{s.t. } & \alpha_1(a_1) + \alpha_1(a_4) = 1, \ \alpha_1(a_2) + \alpha_1(a_3) = 1\\
        & \alpha_1(a_i) \geq 0, \ \forall i \in [4], 
    \end{aligned}
\end{equation}
where the coupled constraints simplified since we are evaluating player one's game with respect to $\alpha_2(a_j) = \half$ for all $j \in [4]$.
Consider the decomposition $\alpha_1 = \alpha_2 = \begin{bmatrix}\half & \half & \half & \half\end{bmatrix}$, we can verify that $\alpha_1$ does not minimize~\eqref{eqn:bimatrix_gne}. Specifically, $\hat{\alpha}_1 = \begin{bmatrix}
    0 & 1 & \half & \half
\end{bmatrix}$ can achieve a lower objective than $\alpha_1$ against $\alpha_2 = \begin{bmatrix}\half & \half & \half & \half\end{bmatrix}$. 
\end{example}
% \begin{proposition}\label{prop:ce_sufficient_0}
%     If $y$ is a correlated equilibrium of an $N$ player game with joint action space $[A]$ and $y(a) > 0$ for all $a \in [A]$, then all of $y$'s normalized decompositions $(\alpha_1,\ldots,\alpha_N)$ are generalized Nash equilibria (Definition~\ref{def:gNE}) of the unnormalized game~\eqref{eqn:ce_individual_opt}. 
% \end{proposition}
% \begin{proof}
% For fully mixed correlated strategies $y$, we prove the proposition's contrapositive: if $(\alpha_1,\ldots,\alpha_N)$ is not the generalized Nash equilibrium of the unnormalized game~\eqref{eqn:ce_individual_opt}, then $y$ is not a correlated equilibria.

% Let $(\alpha_1,\ldots,\alpha_N)$ be a decomposition of $y$. If $(\alpha_1,\ldots,\alpha_N)$ is not a generalized Nash equilibrium, then there exist $i \in [N]$ such that $\alpha_i$ is suboptimal for~\eqref{eqn:ce_individual_opt} with respect to $\alpha_{-i}$. 
% For a fixed $\alpha_{-i}$,~\eqref{eqn:ce_individual_opt} is linear in $\alpha_i$ and independent between $\alpha_i(\cdot, a_{-i})$ for different $a_{-i} \in [A_{-i}]$. Therefore, ~\eqref{eqn:ce_individual_opt} is equivalent to $A_{-i} = \prod_{j\neq i} A_j$ many optimization problems given by
% \begin{equation}\label{eqn:pf_4}
% \begin{aligned}
%     \min_{\alpha_i\in \reals_+^{A}} & \sum_{a_i \in [A_i]} {\ell}_i(a_i, a_{-i}) \alpha_i(a_i, a_{-i})\alpha_{-i}(a_i, a_{-i}), \\
%     \mbox{s.t. } &\sum_{a_i \in [A_i]}\alpha_i(a_i, a_{-i})\alpha_{-i}(a_i, a_{-i}) = \frac{1}{A_{-i}} \ \forall a_{-i} \in [A_{-i}] \\
%     & \alpha_i(a_i, a_{-i}) \geq 0, \ \forall a_i \in [A_i].
% \end{aligned}
% \end{equation}
% If $\alpha_i$ is suboptimal, there exist at least one $a^\star_{-i}$ for which~\eqref{eqn:pf_4} is $\alpha_i$ is suboptimal. We define can define the linear transformation $\beta_i(a_i) = A_i\alpha_i(a_i, a^\star_{-i}) \alpha_{-i}(a_i, a^\star_{-i})$ and $g(a_i) = \ell(a_i, a^\star_{-i})$ such that~\eqref{eqn:pf_4} is equivalent to the following linear program given by
% \begin{equation}\label{eqn:pf_5}
% \begin{aligned}
%     \min_{\beta_i\in \reals_+^{A}} & \frac{1}{A_i}\sum_{a_i \in [A_i]} g(a_i) \beta_i(a_i), \\
%     \mbox{s.t. } &\sum_{a_i \in [A_i]}\beta_i(a_i) = 1,  \ \beta_i(a_i) \geq 0,  \forall a_{i} \in [A_{i}]. 
% \end{aligned}
% \end{equation}
% When $\alpha_i$ is suboptimal for~\eqref{eqn:pf_4}, $\beta_i$ is suboptimal for~\eqref{eqn:pf_5}. Given that~\eqref{eqn:pf_5} is a linear program over the probability simplex $\Delta_i$, $\beta_i$ is optimal if and only if for each $a_i$ such that $\beta_i(a_i) > 0$, $g(a_i) = \min_{\hat{a}_i}g(\hat{a}_i)$. Therefore if $\beta_i$ is suboptimal, there exist $a^\star_i, \hat{a}_i$ such that 
% \[\beta_i(a^\star_i) > 0, \ g(\hat{a}_i) < g(a^\star_i).\]
% Since $\beta_i(a^\star_i)$ is a linear transformation of $\alpha_i$, and $\beta_i(a^\star_i)$ is strictly positive, we can also conclude that there exist $a^\star_i, \hat{a}_i \in [A_i]$ such that 
% \[\alpha_i(a^\star_i, a^\star_{-i}) > 0, \ y(a^\star_i, a^\star_{-i}) > 0, \ \ell(\hat{a}_i, a^\star_{-i}) < \ell(a^\star_i, a^\star_{-i}).\]
% This implies that 
% \[\ell(\hat{a}_i, a^\star_{-i})y(a^\star_i, a^\star_{-i}) > \ell(a^\star_i, a^\star_{-i})y(a^\star_i, a^\star_{-i}).\]  
% We define an alternative probability density $\hat{\beta}$ that is also feasible for~\eqref{eqn:pf_5}, given by
% \[\hat{\beta}(a_i) = \begin{cases}
%     \beta(a_i) & a_i \notin \{a^\star_i, \hat{a}_i\}\\
%     0 & a_i = a^\star_i\\
%     \beta(a^\star_i) + \beta(\hat{a}_i) & a_i = \hat{a}_i
% \end{cases}, \ \forall a_i \in [A_i].\]
% We can evaluate the objective $\sum_{a_i \in [A]}g(a_i)\hat{\beta}_i(a_i)$ as 
% \[\sum_{a_i \in [A]}g(a_i)\hat{\beta}(a_i) = \sum_{a_i \neq a^\star_i}g(a_i)\beta_i(a_i) +g(\hat{a}_i)\beta_i(a^\star_i). \]
% By construction, $\sum_{a_i \in [A]}g(a_i)\hat{\beta}(a_i) < \sum_{a_i \in [A]}g(a_i)\beta_i(a_i)$. We perform the inverse linear transformation to derive 

% Since $\beta_i$ is suboptimal, $\sum_{a_i} {\ell}_i(a_i, a^\star_{-i})\beta_i(a_i) > \sum_{a_i} {\ell}_i(a_i, a^\star_{-i})\beta_i(a_i)\hat{\beta}(a_i)$
% there does not exist $a^\star_i, \hat{a}_i \in [A_i]$ such that 
 

% ,   $\beta_i$ being sub-optimal implies that there exist $a_i, \hat{a}_i \in [A_i]$, such that $\beta_i(a_i) > 0$ and $\ell_i(a_i, a^\star_{-i})$
% we will show that~\eqref{eqn:ce_full_condition} implies that $\alpha_i$ is not the optimal solution 
% When $y$ is not a correlated equilibria, there exist a player $i \in [N]$ and action pair $a^\star_i, \hat{a}_i \in [A_i]$ such that 
% \begin{equation}\label{eqn:ce_full_condition}\sum_{a_{-i}\in[A_{-i}] } \Big(\ell_i(a^\star_i, a_{-i}) - \ell_i({a'}_i, a_{-i})\Big)y(a_i^\star, a_{-i}) > 0,\end{equation}
% Let $(\alpha_1,\ldots,\alpha_N)$ be a decomposition of $y$, we will show that~\eqref{eqn:ce_full_condition} implies that $\alpha_i$ is not the optimal solution 

% s not a generalized Nash equilibirum
% If correlated equilibrium $y$ is strictly positive, then all of its normalized decomposition's $(\alpha_1,\ldots,\alpha_N)$ will all satisfy $\alpha_i(a) > 0$ for all $a\in[A]$ and $i\in[N]$.
% From the correlated equilibrium condition, $\sum_{a_{-i}\in[A_{-i}] } \Big(\ell_i(a_i, a_{-i}) - \ell_i(\hat{a}_i, a_{-i})\Big)y(a_i, a_{-i}) \leq 0$ for all $a_i, \hat{a}_i \in [A_i]$, since each element $ \Big(\ell_i(a_i, a_{-i}) - \ell_i(\hat{a}_i, a_{-i})\Big)$ is multiplied by a strictly positive probability measure within the sum and the sum is less than $0$, this implies . 

    
%  If $y$ is not a correlated equilibrium, then let $a^\star_i, {a'}_i \in [A_i]$ be the actions that violate the correlated equilibrium condition~\eqref{eqn:ce} for player $i$, i.e.,  \begin{equation}\label{eqn:ce_full_condition}\sum_{a_{-i}\in[A_{-i}] } \Big(\ell_i(a^\star_i, a_{-i}) - \ell_i({a'}_i, a_{-i})\Big)y(a_i^\star, a_{-i}) > 0,\end{equation}
%  then we can construct $\hat{\alpha}_i$ such that $(\hat\alpha_i, \alpha_{-i})$ is a feasible decomposition of $y$ and achieves a lower objective value for~\eqref{eqn:ce_individual_opt}.

% Let $\beta(a_i, a_{-i}) = \alpha_i(a^\star_i, a_{-i})\frac{\alpha_{-i}(a^\star_i, a_{-i})}{\alpha_{-i}(a_i, a_{-i})}$, we construct the new feasible $\hat{\alpha}_i$ as follows 
% \[\hat{\alpha}_{i}(a_i, a_{-i}) = \begin{cases}
%     \alpha_i(a_i, a_{-i}) & a_i \notin \{a^\star_i, a'_i\}\\
%     \alpha_i(a_i, a_{-i}) +\beta(a_i, a_{-i}) & a_i= a'_i\\
%     0 & a_i  = a^\star_i
% \end{cases}.\]
% The objective value in~\eqref{eqn:ce_individual_opt} achieved by $\hat{\alpha}$ for player $i$ is given by $\sum_{a \in [A]}\hat{\alpha}(a)\ell_i(a)$ and can be partitioned as follows:
% \begin{multline}\label{eqn:new_obj_val} %\sum_{a \in [A]}\prod_{i\in[N]}\hat{\alpha}_i(a)\ell_i(a) & =
%      \sum_{a_i \notin \{a_i^\star, a'_i\}} \sum_{a_{-i} \in [A_{-i}]} \alpha_i(a_i, a_{-i}) \ell_i(a_i, a_{-i}) \\
%      + \sum_{a_{-i}\in [A_{-i}]} \alpha_{i}(a^\star_i, a_{-i})\alpha_{-i}(a^\star_i, a_{-i})\ell_i(a'_i, a_{-i}) \\
%      + \sum_{a_{-i}\in [A_{-i}]}\alpha_i(a_i', a_{-i})\alpha_{-i}(a'_i, a_{-i})\ell_i(a'_i, a_{-i}). 
% \end{multline}
% In comparison, the objective value achieved by $\alpha$ is given by $\sum_{a \in [A]}{\alpha}(a)\ell_i(a)$ and can be partitioned as 
% \begin{multline}\label{eqn:orig_obj_val} 
% \sum_{a_i \notin \{a_i^\star, a'_i\}} \sum_{a_{-i} \in [A_{-i}]} \alpha(a_i, a_{-i}) \ell_i(a) \\
% + \sum_{a_{-i} \in [A_{-i}]}\alpha_i(a^\star_i, a_{-i})\alpha_{-i}(a^\star, a_{-i})\ell_i(a^\star_i, a_{-i}) \\
% +\sum_{a_{-i}\in [A_{-i}]}\alpha_i(a_i', a_{-i})\alpha_{-i}(a'_i, a_{-i})\ell_i(a'_i, a_{-i}). 
% \end{multline}
% The only difference between the objectives in~\eqref{eqn:new_obj_val} and~\eqref{eqn:orig_obj_val} occurs in the second term, whose difference is given by~\eqref{eqn:ce_full_condition}. Therefore, we conclude that $\sum_{a \in [A]}\hat{\alpha}(a)\ell_i(a) < \sum_{a \in [A]}{\alpha}(a)\ell_i(a)$. Let $\hat{y} = \hat{\alpha}_i\circ\alpha_{-i}$, by construction, $\ones^\top \hat{y} =  \ones^\top y = 1$, $\hat{\alpha}_i \geq 0$. Therefore $(\hat{\alpha}_i, \alpha_{-i})$ is feasible for~\eqref{eqn:ce_individual_opt}, and $\hat{\alpha}_i$ achieves a smaller objective in~\eqref{eqn:ce_individual_opt} than $\alpha_i$. Therefore, $\alpha_i$ cannot be the optimal for~\eqref{eqn:ce_individual_opt} with respect to $\alpha_{-i}$. 
% \end{proof}
From Propositions~\ref{prop:ce_necessary}, we can say that if the generalized Nash equilibrium of~\eqref{eqn:ce_individual_opt} is strictly positive,  then their product $y$ is a strictly positive correlated equilibria of the original normalized game. A natural follow up question is then when do strictly positive correlated strategies exist? We explore this in the following section using entropy-regularizations. 








==> contents/entropy_CE_new_version.tex <==
\section{Entropy-Regularized Correlated Equilibria}\label{sec:entropy_reg_equilibria}
A coupled optimization framework for correlated equilibria expands the set of applicable techniques for analyzing correlated equilibrium. In this section, we demonstrate how entropy regularization can be applied to the unnormalized  game and how to find a closed-form solution to the entropy-regularized unnormalized distribution game. 

We consider the entropy-regularized counterpart of the unnormalized distribution game~\eqref{eqn:ce_individual_opt}, where each player solves the optimization problem given by 
\begin{equation}\label{eqn:ce_entropy_reg}
\begin{aligned}
  \min_{\alpha_i\in \reals_+^{A}}& \sum_{a \in [A]} \Bigg({\ell}_i(a)+ \frac{1}{\lambda_i}\Big(\log\big({\alpha_i}(a)\big) - 1\Big)\Bigg) \alpha_i(a)\alpha_{-i}(a) \\
\mbox{s.t. } & \sum_{a_i \in [A_i]}(\alpha_1\circ\ldots\circ\alpha_N)(a_i, a_{-i}) = \frac{1}{A_i},  \ \forall a_{-i} \in [A_{-i}], \\
&\alpha_i \geq 0. %\ones^\top \alpha = \ones^\top,  
\end{aligned}
\end{equation}
Here, $\lambda_i \geq 0$, $\lambda_i\in \reals$ denotes the magnitude of entropy regularization. The total entropy of the correlated strategy $y = \alpha_1\circ\ldots\circ\alpha_{N}$ is given by $\sum_{a\in[A]} y(a)\log({y(a)})$, such that $\sum_{a\in[A]} y(a)\log({\alpha_i}) $ is equivalent to player $i$'s contribution to the total entropy.  Given two unnormalized measures that achieve equal cost $\sum_{a \in [A]} {\ell}_i(a) \alpha_i(a) \alpha_{-i}(a)$,~\eqref{eqn:ce_entropy_reg} will favor the measure with greater entropy. Thus, the optimal strategy produced by~\eqref{eqn:ce_entropy_reg} is less sensitive to sporadic modeling imperfections than those produced by~\eqref{eqn:ce_individual_opt}.
\begin{remark}
    Since~\eqref{eqn:ce_entropy_reg} has a strongly convex objective, a player-wise convex shared constraint, the generalized Nash equilibrium of the game can be characterized by the optimal solutions of the coupled KKT conditions~\cite{dreves2011solution}. 
\end{remark}
\begin{remark}
In applications of game-theoretic equilibrium, player costs and transitions are often obtained from noisy and imperfect data. When faced with such modeling inaccuracy data, it is in the player's best interest to seek strategies that not only optimize their expected cost but also maximize the entropy over the action space. 
Entropy regularization has been used in single agent reinforcement learning and Nash equilibrium to find optimal policies that are robust to modeling inaccuracies and `unforseen changes in the environment'~\cite{guan2020learning,savas2019entropy}. The Nash equilibrium of entropy regularized games are also known as \emph{logit quantal response equilibrium}~\cite{mckelvey1995quantal} and are an important tool for approximating Nash equilibria in multi-agent reinforcement learning for policy-based gradient methods learning~\cite{cen2021fast}. Furthermore, the logit quantal response equilibrium is shown to be a more robust equilibrium model than Nash equilibrium for games models involving human players~\cite{alsaleh2022road}.
\end{remark}
We can show that the entropy-regularized unnormalized distribution game has closed-form solutions.
% , which can be used in conjunction with Corollary~\ref{cor:approx_ce} to approximate the correlated equilibrium while incurring significantly less computation complexity. 
\begin{proposition}\label{prop:entropy_reg}
In the entropy-regularized unnormalized game where each player solves~\eqref{eqn:ce_entropy_reg}, there exists a generalized Nash equilibrium $(\alpha_1,\ldots,\alpha_N)$, where $\alpha_i$ is given by
    \begin{equation}\label{eqn:gNE_entropy_solution}
        \alpha_{i}(a) = \frac{\exp\big(-\lambda_i\ell_i(a)\big)}{\Big(\sum_a\exp\big(-\sum_j\lambda_j\ell_j(a)\big) \Big)^{\lambda_i/ \sum_{j}\lambda_j}}, \ \forall i, a \in [N]\times[A].
    \end{equation}
\end{proposition}
\begin{proof}
We assign the Lagrange multipliers $\sigma_i(a_{-i}) \in \reals$ to the constraint 
 $\sum_{a_i \in [A_i]}(\alpha_1\circ\ldots\circ\alpha_N)(a_i, a_{-i}) = \frac{1}{A_i},  \ \forall a_{-i} \in [A_{-i}]$ and $\mu_i(a) \in \reals_+$ to the constraints $\alpha_i(a) \geq 0$, for all $a \in [A]$. The KKT conditions of~\eqref{eqn:ce_entropy_reg} are given by 
\begin{equation}~\label{eqn:kkt_condition}
    \begin{aligned}
        0 =&  \big(\ell_i(a) + \frac{1}{\lambda_i}\log\big(\alpha_i(a)\big)+\sigma_i(a_{-i})\big)\alpha_{-i}(a)- \mu_i(a), \ \forall a \in [A], \\
        \frac{1}{A_{-i}} = & \sum_{a_i \in [A_i]}(\alpha_1\circ\ldots\circ\alpha_N)(a_i, a_{-i}), \ \forall a_{-i} \in [A_{-i}],\\
        0 \leq & \alpha_i(a), 0 \leq \mu_i(a), 0 =\alpha_i(a) \mu_i(a),\ \forall a \in [A].
    \end{aligned}
\end{equation}
When $\alpha_{-i}(a) > 0$ and $\alpha_i(a) > 0$, the first KKT condition reduces down to $0 = \ell_i(a) + \frac{1}{\lambda_i}\log(\alpha_i(a)) + \sigma_i(a_{-i})$. We can solve for $\alpha_i(a)$ as
\begin{equation}\label{eqn:pf_5}
    \alpha_i(a) = \exp\Big(-\lambda_i\big(\sigma_i(a_{-i})+\ell_i(a)\big)\Big).
\end{equation}
For each joint action $a\in [A]$, the product $(\alpha_1\circ\ldots\circ\alpha_N)(a)$ is given by 
\begin{equation}\label{eqn:pf_6}
 (\alpha_1\circ\ldots\circ\alpha_N)(a) = \exp\Big(-\sum_{i}\lambda_i\sigma_i(a_{-i}) - \sum_i\lambda_i\ell_i(a)\Big).   
\end{equation}
From primal feasibility of the KKT conditions, $\sum_{a_{-i}}\sum_{a_i} (\alpha_1(a)\circ\ldots\circ\alpha_N)(a_i, a_{-i}) = 1$. We combine this with~\eqref{eqn:pf_6} to derive
    \begin{equation}\label{eqn:pf_condition_2}
        \sum_{a} \exp\big(-\sum_i \lambda_i\sigma_i(a_{-i})\big) \exp\big(-\sum_{i}\lambda_i\ell_i(a)\big) = 1.
    \end{equation}
    Let $\lambda_N = \sum_{i}\lambda_i$ and $\sigma_i\big(a_{-i}\big) = \sigma$ for all $a_{-i} \in [A_{-i}]$ and $i \in [N]$. 
    We can then solve for $\exp(\sigma)$ in~\eqref{eqn:pf_condition_2} as
    \[\exp(\sigma) =  \Big(\sum_a \exp\big(-\sum_i\lambda_i \ell_i(a)\big)\Big)^{-1/\lambda_N}.\]
    Let $\beta_i(a) = \exp\big(-\lambda_i\ell_i(a)\big)$, each $\alpha_i(a)$~\eqref{eqn:pf_5} is given by 
    \begin{equation}
        \alpha_{i}(a) = \frac{\beta_i(a)}{\Big(\sum_a\prod_{j}\beta_j(a)\Big)^{\lambda_i/\lambda_N}}.
    \end{equation}
    When $\lambda_i, \ell_i(a)$ are finite, $\alpha_i(a) >0 $ for all $i, a \in [N]\times[A]$. Therefore $\alpha_1,\ldots,\alpha_N$ satisfy the KKT conditions and are the optimal solutions to the unnormalized game.
    % We will construct some Lagrange multipliers for $\alpha_1,\ldots\alpha_N$~\eqref{eqn:gNE_entropy_solution} and show that they satisfy the KKT conditions. 
\end{proof}
% \noindent\textbf{Modified equilibrium condition}. With the additional entropy penalty, the generalized Nash equilibrium of~\eqref{eqn:ce_entropy_reg} satisfies an \emph{entropy-regularized} version of the correlated equilibrium condition~\eqref{eqn:ce}. 
\begin{proposition}[Entropy-regularized optimality]\label{prop:entropy_ce_condition}
For strictly positive unnormalized distributions, $(\alpha^{\star}_1,\ldots,\alpha^{\star}_N)$ is a generalized Nash equilibrium of the entropy-regularized unnormalized distribution game~\eqref{eqn:gNE_entropy_solution} if for every $i \in [N]$ and $a_{-i} \in [A_{-i}]$,
\begin{multline}\label{eqn:entropy_reg_ce_like}
    y(a_i, a_{-i})\Big(\hat{\ell}_i(a_i, a_{-i})  - \hat{\ell}_i(a'_i, a_{-i})\Big)  \leq 0, \ \forall a_i, a'_i \in [A_i], 
\end{multline}
where $\hat{\ell}_i(a_i, a_{-i}) = \ell_i(a_i, a_{-i}) + \frac{1}{\lambda_i}\log\Big(\alpha^{\star}_i(a_i, a_{-i})\Big)$.
\end{proposition}
\begin{proof}
We note that from~\cite{dreves2011solution}, the coupled KKT conditions of~\eqref{eqn:ce_entropy_reg} are necessary for the optimality. We assign the Lagrange multipliers $\mu_i(a)$ for the constraint $\alpha_i(a) \geq 0$, for all $i,a \in [N]\times[A]$, and $\sigma_{i}$ for the constraint $\ones^\top(\alpha_1\circ\ldots\circ\alpha_N) = 1$, and consider the optimal Lagrange multipliers $\mu^{\star}_{i}$ and $\sigma_{i}^{\star}$ for the optimal solution $\alpha_{1}^{\star},\ldots,\alpha_{N}^{\star}$. From the corresponding KKT conditions, we derive the following
\begin{multline}
    [\alpha^{\star}_{-i}(a)\Big(\ell_i(a)+ \frac{1}{\lambda_i}\log(\alpha^{\star}_i(a))\ + \frac{1}{\lambda_i}\sigma^{\star}_{i} \Big)  + \mu_{i}^{\star} =  0, \\
    \forall i \in [N], a \in [A].
\end{multline}
Since all $\alpha^{\star}_i(a) > 0$, $\mu_i(a) = 0$ and the above inequality becomes equality, such that for all $a'_i \in [A_i]$, $\frac{1}{\lambda_i}\sigma^{\star}_{i} = -\ell_i(a'_i, a_{-i}) - \frac{1}{\lambda_i}\log(\alpha^{\star}_i(a'_i, a_{-i}))$. Let $\hat{\ell}_i(a_i, a_{-i}) = \ell_i(a'_i, a_{-i}) + \frac{1}{\lambda_i}\log(\alpha^{\star}_i(a'_i, a_{-i}))$, then~\eqref{eqn:entropy_reg_ce_like} holds for all $a_i, a'_i \in [A_i]$.
\end{proof}
We note that while Proposition~\ref{prop:entropy_reg} provides one possible solution for the entropy-regularized unnormalized game~\eqref{eqn:ce_entropy_reg}, other generalized Nash equilibria exist. In particular, each generalized Nash equilibrium approximates the un-regularized correlated equilibria of the normal form game~\eqref{eqn:ce_individual_opt}. 
\begin{corollary}[$\epsilon$-correlated equilibrium]\label{cor:approx_ce}
Given a strictly positive normalized decomposition $\alpha_1,\ldots,\alpha_N$ that is the generalized Nash equilibrium of an entropy-regularized unnormalized distribution game, their product  $y = \alpha_1\circ\ldots\circ\alpha_N$ is an $\epsilon$-correlated equilibria---i.e., for all $i \in [N]$, 
   \begin{equation}\label{eqn:theoretial_bound}
       \sum_{a_{-i}} y(a_i, a_{-i})\Big(\ell_i(a_i, a_{-i}) - \ell_i(\hat{a}_i, a_{-i})\Big) \leq \frac{\epsilon}{\lambda_i}, \ \forall a_i, \hat{a}_i \in [A_i]. 
   \end{equation}
    where  
    \[\epsilon = \max_{a_i, \hat{a}_i \in[A_i]} \log\Big(\alpha_i(a_i, a_{-i})/\alpha_i(\hat{a}_i, a_{-i})\Big). \]
   \end{corollary}
\begin{proof}
In Proposition~\ref{prop:entropy_ce_condition}'s proof, we derived the coupled KKT conditions~\eqref{eqn:kkt_condition} of the entropy-regularized unnormalized game. When $\alpha_i(a) > 0$ for all $(i,a)\in [N]\times[A_i]$, the following holds:
\begin{equation}
    \ell_i(a) + \frac{1}{\lambda_i}\log(\alpha_i(a)) + \sigma_i(a_{-i}) = 0, \forall a \in [A].
\end{equation}
Then for any $a_i, a'_i \in [A_i]$, their cost difference for the same $a_{-i}$ is given by 
\begin{equation}\label{eqn:pf_7}
   \ell_i(a_i, a_{-i}) - \ell_i(a'_i, a_{-i}) = \frac{1}{\lambda_i}\log(\frac{\alpha_i(a_i, a_{-i})}{\alpha_i(a'_i, a_{-i})}).
   \end{equation}
We multiply~\eqref{eqn:pf_7} by $y(a_i, a_{-i})$ and sum over $a_{-i} \in [A_{-i}]$ to obtain
\begin{multline}\label{eqn:pf_7}
   \sum_{a_{-i}} y(a_i, a_{-i})\Big(\ell_i(a_i, a_{-i}) - \ell_i(a'_i, a_{-i})\Big) = \\
   \frac{1}{\lambda_i}\sum_{a_{-i} \in [A_{-i}]} y(a_i, a_{-i})\log(\frac{\alpha_i(a_i, a_{-i})}{\alpha_i(a'_i, a_{-i})}).
   \end{multline}
Let $\max_{a, {a'}\in[A]} \log(\frac{\alpha_i(a)}{\alpha_i(a')}) = \epsilon_i$. It follows that
\begin{multline}
    \sum_{a_{-i} \in [A_{-i}]} y(a_i, a_{-i})\log(\frac{\alpha_i(a_i, a_{-i})}{\alpha_i(a'_i, a_{-i})}) \leq \sum_{a \in [A]} y(a)\epsilon_i \leq \epsilon_i.
\end{multline}
We can then conclude the proposed statement~\eqref{eqn:theoretial_bound}. 
\end{proof}


